Intent-Based Orchestration for Application Relocation in a 5G Cloud-native Platform

The need of mobile network operators for cost-effectiveness is driving 5G and beyond networks towards highly flexible and agile deployments to adapt to dynamic and resource-constrained scenarios while meeting a myriad of user network stakeholders' requirements. In this setting, we consider that zero-touch orchestration schemes based on cloud-native deployments equipped with end-to-end monitoring capabilities provide the necessary technology mix to be a solution candidate. This demonstration, built on top of an end-to-end cloud-native 5G experimental platform with over-the-air transmissions, shows how dynamic orchestration can relocate container-based end-user applications to fulfil intent-based requirements. Accordingly, we provide an experimental validation to showcase how the platform enables the desired flexible and agile 5G deployments.

==> sections/evaluation.tex <==
\section{Use case evaluation} \label{section:evaluation}

The evaluation/observation steps go here.

==> sections/use_case.tex <==
\section{Use case scenario} \label{section:use_case}

The use case goes here.

\begin{figure*}[h!]
	\centering
	\includegraphics[width=1\textwidth]{img/scenario.png}
	\caption{Experimental scenario under demonstration.}
	\label{fig:scenario}
\end{figure*}

\textbf{*** INTERNAL NOTES TO BE CONVERTED :) ***}

\textbf{IDEA}: present a demo on a use case where we demonstrate the usage of an orchestrator that automatically adapts to the network and UE requirements given a K8s-based infra. This suits perfectly to 5G automatization concept.

\textbf{CONTRIBUTIONS}: A tangible open source solution for \textit{slice} orchestration in a cloud-native 5G network. We put together buzzword concepts like 5G core (Open5GS), edge (including UPF close to the UE), orchestration of resources to match service demands, and end-to-end monitoring of both infra and networking metrics. Besides, we depict the architecture of our solution, which includes CLEAR definitions of what things are (e.g., we explain a realization of an intent, and the orchestration process).

\textbf{SCENARIO}: Assume an APP/Service (e.g., virtual reality) that imposes certain requirements on latency and reliability (meaning that it is needed that the node hosting the APP is always below a certain CPU threshold to avoid overloading). We emulate such an APP through an `nginx` container. Notice that this APP is dummy and could be anything. The APP should be running in some worker node within the infra implementation (see Fig.~\ref{fig:scenario}), composed of the RAN (gNB), Radio/Regional edge (with three worker nodes/servers), and cloud (with also three nodes/servers). Both radio/regional edge and cloud servers compose a Kubernetes cluster. Monitoring system based on Prometheus provides end-to-end monitoring (including latency and CPU).

The idea is to grant that the requirements on latency and CPU of such an APP are granted. In order to do so, we rely on a Python orchestrator that periodically checks the corresponding metrics in each node and relocates the APP whenever needed. In particular, we define the APP requirements as an intent, composed of conditions. In this case, conditions are related to latency ($<$ 3 ms) and CPU usage of the node running the APP ($<$ 50\%).  Accordingly, the orchestrator will try to locate the APP in a node fulfilling such conditions. Apart from the intent, the orchestrator takes as input general configuration parameters (e.g., Kubernetes authentication).

Besides, as network/infra admins, say we want to give priority for deploying the APP in the core, in worker-5. That is, the orchestrator takes into account the requirements of two tenants (the APP provider and the infra provider). So, APP is deployed by default in worker-5. Such default node is indicated in a configuration file (`config.yaml`) for the Python script, as well as other parameters like the corresponding deployment or namespace.

The orchestrator periodically checks if the node running the APP is fulfilling the required intent conditions (latency and CPU). This is done by scraping metrics from Prometheus, which are exposed in every k8s node. Should the node running the APP no longer fulfill the requirements, the orchestrator must trigger a relocation of the APP to another node.
To force a relocation of the APP, we emulate an addition of 3 ms delay in the interface of worker-5. Also, we stress CPU usage at edge node worker-3. This way, the latency condition of worker-5 is no longer achieved, as well as the CPU usage condition of worker-3. Accordingly, the other edge node worker-2 is the only candidate remaining to run the APP, and a deployment patch is triggered, terminating the APP at the original node, and instantiating it in the new node.
Finally, the orchestrator must periodically check whether the node with priority (worker-5) fulfills the intent conditions. If so, a new relocation must be triggered from the edge node towards the core node.


\textbf{ABOUT 5G REALIZATION}: we must demonstrate previous scenario but adding a 5G flavor. Meaning, we will deploy a 5G core in the cloud, but deploy the UPF at the edge. This way, the latency to edge is less than to the core, as expected in the real world. \textbf{FUTURE}: Would be great to implement to UPFs (one in edge and other in core) and let the APP communicate the 5G network what is the most convenient one for the UE, so a PDU Session is terminated/started, but I think this is not needed at all for this demo.

\textbf{WHAT WE WILL SHOW}: Essentially, a figure displaying the latency (between the Simbox UE and APP) in different stages of the experiment. We will define events (e.g., traffic jam in the transport network resulting in an increase of latency to the core). Result should be something like Fig.~\ref{fig:latency}. We can also think about other experiment steps to display the effect of CPU as well.

\begin{figure}[h!]
	\centering
	\includegraphics[width=0.495\textwidth]{img/latency.png}
	\caption{Latency.}
	\label{fig:latency}
\end{figure}
